An Electronic Compendium of Extreme Functions for the Gomory--Johnson Infinite Group Problem

In this note we announce the availability of an electronic compendium of extreme functions for Gomory--Johnson's infinite group problem. These functions serve as the strongest cut-generating functions for integer linear optimization problems. We also close several gaps in the literature.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=extreme-notes

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

EXTREME_GRAPHICS_SOURCES=

EXTREME_GENERATED_GRAPHICS=$(EXTREME_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(EXTREME_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(EXTREME_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(EXTREME_GRAPHICS_SOURCES:%.fig=%.pstex)

EXTREME_SOURCES=Makefile $(MAINTEXFILE).tex $(EXTREME_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex example-sage-session.txt igp-survey.aux

EXTREME_STYLES = bhk-style.tex

EXTREME_GRAPHICS=$(EXTREME_GENERATED_GRAPHICS)		\
	bccz_counterexample.pdf				\
	bhk_irrational.pdf				\
	chen_3_slope_not_extreme-covered_intervals.pdf	\
	chen_3_slope_not_extreme-perturbation-1.pdf	\
	chen_4_slope.pdf				\
	dg_2_step_mir.pdf				\
	dg_2_step_mir_limit.pdf				\
	dr_projected_sequential_merge_3_slope.pdf	\
	drlm_2_slope_limit.pdf				\
	drlm_3_slope_limit.pdf				\
	drlm_backward_3_slope-2d_diagram.pdf		\
	drlm_backward_3_slope.pdf			\
	gj_2_slope.pdf					\
	gj_2_slope_repeat.pdf				\
	gj_forward_3_slope.pdf				\
	gmic.pdf					\
	hildebrand_2_sided_discont_1_slope_1.pdf	\
	hildebrand_2_sided_discont_2_slope_1.pdf	\
	hildebrand_5_slope_22_1.pdf			\
	hildebrand_discont_3_slope_1.pdf		\
	kf_n_step_mir-lemma5_1.pdf			\
	kf_n_step_mir.pdf				\
	ll_strong_fractional.pdf			\
	rlm_dpl1_extreme_3a-2d_diagram.pdf		\
	rlm_dpl1_extreme_3a.pdf

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(EXTREME_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(EXTREME_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

EXTREME_SOURCES_AND_MORE=$(EXTREME_SOURCES) $(EXTREME_GRAPHICS) $(EXTREME_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(EXTREME_SOURCES)					\
		$(EXTREME_GRAPHICS)					\
		$(EXTREME_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

